Statistical Model Checking for Stochastic Hybrid Systems

This paper presents novel extensions and applications of the UPPAAL-SMC model checker. The extensions allow for statistical model checking of stochastic hybrid systems. We show how our race-based stochastic semantics extends to networks of hybrid systems, and indicate the integration technique applied for implementing this semantics in the UPPAAL-SMC simulation engine. We report on two applications of the resulting tool-set coming from systems biology and energy aware buildings.

==> eptcsdata.tex <==
\providecommand{\firstpage}{122}
\providecommand{\publicationstatus}{Ezio Bartocci and Luca Bortolussi (Eds.): HSB 2012\\
EPTCS 92, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.92.9}{10.4204/EPTCS.92.9}}

